Explain-then-Translate: An Analysis on Improving Program Translation with Self-generated Explanations

This work explores the use of self-generated natural language explanations as an intermediate step for code-to-code translation with language models. Across three types of explanations and 19 programming languages constructed from the MultiPL-E dataset, we find the explanations to be particularly effective in the zero-shot case, improving performance by 12% on average. Improvements with natural language explanations are particularly pronounced on difficult programs. We release our dataset, code, and canonical solutions in all 19 languages.

==> prompts/main-combined-old.tex <==
% \begin{frame*}
% \begin{tcbraster*}[raster columns=2, raster valign=top, raster equal height=rows]
\begin{figure*}[!ht]
    % \input{prompts/main-nl-code}  % skipping to save space and less relevant to our work
    \input{prompts/main-direct}
    \input{prompts/main-exp}
    \caption{Compared to \textbf{direct} code translation prompt, \textbf{exp} (ours) prompts models to explain the code before translating. Example explanations for \textbf{exp-lbl} and \textbf{exp-lbl-d} in Apx~\ref{apx:full-prompt},~\ref{apx:exp-qualitative}}
    \label{fig:prompt-main}
    % \dbltextfloatsep=0em
\end{figure*}
% \end{tcbraster*}
% \end{frame*}

==> prompts/main-direct-old.tex <==
\begin{tcolorbox}[colback=white,title=Code-to-Code (baseline): direct]
\vspace{-\baselineskip}
\begin{lstlisting}[style=text]
Please translate the following Python code to JavaScript?
\end{lstlisting}\vspace{-\baselineskip}
\begin{lstlisting}[style=prompt]
(*@\codehl{\#\#\# Python version}@*)
from typing import List

def unique(l: List[int]) -> List[int]:
    return sorted(list(set(l)))
(*@\codehl{\#\#\# JavaScript version}@*)
\end{lstlisting}\vspace{-\baselineskip}
\begin{lstlisting}[style=js]
function unique(l){
(*@\inserthl{<insert JavaScript completion here>}@*)
\end{lstlisting}\vspace{-\baselineskip}
\end{tcolorbox}

==> prompts/main-direct.tex <==
\begin{tcolorbox}[colback=white,title=Standard Translation (baseline): direct]
\vspace{-\baselineskip}
\begin{lstlisting}[style=text]
Please translate the following Python code to JavaScript?
\end{lstlisting}\vspace{-\baselineskip}
\begin{lstlisting}[style=prompt]
(*@\codehl{\#\#\# Python version}@*)
def largest_divisor(n: int) -> int:
    for i in reversed(range(n)):
        if n % i == 0:
            return i
(*@\codehl{\#\#\# R version}@*)
\end{lstlisting}\vspace{-\baselineskip}
\begin{lstlisting}[style=js]
largest_divisor <- function(n) {
  (*@\inserthl{for (i in rev(seq(}@*)(*@\codehlerr{n}@*)(*@\inserthl{))) \{ }@*)
    (*@\inserthl{if (n \%\% i == 0) \{ }@*)
      (*@\inserthl{return(i)}@*)
    (*@\inserthl{\} }@*)
  (*@\inserthl{\} }@*)
(*@\inserthl{\}}@*)   // Translation is incorrect!
\end{lstlisting}\vspace{-\baselineskip}
\end{tcolorbox}

==> prompts/main-exp-old.tex <==
\begin{tcolorbox}[colback=white,title=Code-to-Code (ours): exp]
\vspace{-\baselineskip}
\begin{lstlisting}[style=text]
Can you explain what this Python program does with a couple of sentences? The goal with the explanation, is so that a reader can easily rewrite the program in JavaScript.
\end{lstlisting}\vspace{-\baselineskip}
\begin{lstlisting}[style=prompt]
(*@\codehl{\#\#\# Python version}@*)
from typing import List

def unique(l: List[int]) -> List[int]:
    return sorted(list(set(l)))
(*@\codehl{\#\#\# Explanation}@*)
This(*@\inserthl{<insert exp completion here>}@*)
(*@\codehl{\#\#\# JavaScript version}@*)
\end{lstlisting}\vspace{-\baselineskip}
\begin{lstlisting}[style=js]
function unique(l){
(*@\inserthl{<insert JavaScript completion here>}@*)
\end{lstlisting}\vspace{-\baselineskip}
\end{tcolorbox}

==> prompts/main-exp.tex <==
\begin{tcolorbox}[colback=white,title=Explain-then-Translate (ours): exp]
\vspace{-\baselineskip}
\begin{lstlisting}[style=text]
Can you explain what this Python program does with a couple of sentences? The goal with the explanation, is so that a reader can easily rewrite the program in R.
\end{lstlisting}\vspace{-\baselineskip}
\begin{lstlisting}[style=prompt]
(*@\codehl{\#\#\# Python version}@*)
def largest_divisor(n: int) -> int:
    for i in reversed(range(n)):
        if n % i == 0:
            return i
(*@\codehl{\#\#\# Explanation}@*)
This (*@\inserthl{function takes an integer `n` and returns the largest divisor of `n`. It does this by iterating over all integers from `n-1` down to `1` and checking if `n` is divisible by each integer. If it is, the function returns that integer. If no divisor is found, the function returns `1`.}@*)
(*@\codehl{\#\#\# R version}@*)
\end{lstlisting}\vspace{-\baselineskip}
\begin{lstlisting}[style=js]
largest_divisor <- function(n) {
  (*@\inserthl{for (i in rev(seq\_len(}@*)(*@\codehlerr{n - 1}@*)(*@\inserthl{))) \{ }@*)
    (*@\inserthl{if (n \%\% i == 0) \{ }@*)
      (*@\inserthl{return(i)}@*)
    (*@\inserthl{\} }@*)
  (*@\codehlerr{return(1)}@*)
(*@\inserthl{\}}@*)   // Translation is correct!
\end{lstlisting}\vspace{-\baselineskip}
\end{tcolorbox}

==> prompts/main-nl-code.tex <==
\begin{tcolorbox}[toprule at break=0pt,bottomrule at break=0pt,colback=white,title=NL-to-Code (MultiPL-E)]
\vspace{-\baselineskip}
\begin{lstlisting}[style=js]
//Return sorted unique elements in an array
// >>> unique([5, 3, 5, 2, 3, 3, 9, 0, 123])
// [0, 2, 3, 5, 9, 123]
function unique(l){
(*@\inserthl{<insert JavaScript completion here>}@*)
\end{lstlisting}\vspace{-\baselineskip}
\end{tcolorbox}
